Statistical Methods for Investigating the Cosmic Ray Energy Spectrum

Two separate statistical tests are described and developed in order to test un-binned data sets for adherence to the power-law form. The first test employs the TP-statistic, a function defined to deviate from zero when the sample deviates from the power-law form, regardless of the value of the power index. The second test employs a likelihood ratio test to reject a power-law background in favor of a model signal distribution with a cut-off.

==> doit <==
#! /bin/sh
#Script to create the note and open the PDF
#powerlaw.
echo  "\n**************************************************"
echo  "La/Bib-Texing $1."
echo  "**************************************************"
latex $1.tex
bibtex $1 ###
latex $1.tex
latex $1.tex

echo  "\n**************************************************"
echo  "Converting $1.dvi -> $1.pdf"
echo  "**************************************************"
dvipdf $1.dvi

#echo  "Converting $1.ps -> $1.pdf"
#ps2pdf $1.ps
echo  "\n**************************************************"
echo  "Opening $1.pdf"
echo  "**************************************************"
#/usr/local/Adobe/Acrobat7.0/bin/acroread $1.pdf &
evince $1.pdf &

